Fair Division via the Cake-Cutting Share

In this paper, we consider the classic fair division problem of allocating $m$ divisible items to $n$ agents with linear valuations over the items. We define novel notions of fair shares from the perspective of individual agents via the cake-cutting process. These shares generalize the notion of proportionality by taking into account the valuations of other agents via constraints capturing envy. We study what fraction (approximation) of these shares are achievable in the worst case, and present tight and non-trivial approximation bounds as a function of $n$ and $m$. In particular, we show a tight approximation bound of $\Theta(\sqrt{n})$ for various notions of such shares. We show this bound via a novel application of dual fitting, which may be of independent interest. We also present a bound of $O(m^{2/3})$ for a strict notion of share, with an almost matching lower bound. We further develop weaker notions of shares whose approximation bounds interpolate smoothly between proportionality and the shares described above. We finally present empirical results showing that our definitions lead to more reasonable shares than the standard fair share notion of proportionality.

==> omitted_proofs.tex <==








  


==> other.tex <==
\section{Other Properties}
CCS and EFS, along with our algorithm, exhibit additional properties beyond {\em proportionality} and {\em envy-freeness}.

\km{I don't understand the text below. Can we connect our properties to those in \citet{Babaioff}?}

\paragraph{truthfulness} 
The incentive for truthful reporting ensures that an agent cannot obtain a better contract by misreporting their valuation vector. As discussed in lemma 2.3, the CCS value for any agent is the optinal solution of the LP. Untruthful reporting of valuation vector would result in an non-optimal solution. Similarly, EFS also upholds the property of truthfulness.








